ISAC Channel Modelling -- Perspectives from ETSI

Integrated Sensing and Communications (ISAC) is defined as one of six usage scenarios in the ITU-R International Mobile Telecommunications (IMT) 2030 framework for 6G. ISAC is envisioned to introduce the sensing capability into the cellular network, where sensing may be obtained using the cellular radio frequency (RF) signals with or without additional auxiliary sensors. To enable ISAC, specification bodies such as European Telecommunications Standards Institute (ETSI) and Third Generation Partnership Project (3GPP) have already started to look into detailed ISAC use cases, their requirements, and the channel models and evaluation methodologies that are necessary to design and evaluate ISAC performance. With focus on the channel model, the current communication-centric channel models like those specified in 3GPP technical report (TR) 38.901 do not cover the RF signals interactions between the transmitter, target object, receiver and their surrounding environment. To bridge this gap, 3GPP has been looking into the basic changes that are necessary to make to their TR38.901 channel model with focus on selected use cases from the 3GPP SA1 5G-Advanced feasibility study. In parallel, ETSI ISAC Industry Specification Group (ISG) has been studying the more advanced ISAC channel modelling features that are needed to support the variety of ISAC use cases envisioned in 6G. In this paper, we present the baseline and advanced features developed thus far in 3GPP and ETSI ISAC ISG, respectively, towards a comprehensive view of the ISAC channel model in 6G.

==> Sections/Section3.tex <==
\section{ISAC channel model use case scenarios}
